VitaLITy: Promoting Serendipitous Discovery of Academic Literature with Transformers & Visual Analytics

There are a few prominent practices for conducting reviews of academic literature, including searching for specific keywords on Google Scholar or checking citations from some initial seed paper(s). These approaches serve a critical purpose for academic literature reviews, yet there remain challenges in identifying relevant literature when similar work may utilize different terminology (e.g., mixed-initiative visual analytics papers may not use the same terminology as papers on model-steering, yet the two topics are relevant to one another). In this paper, we introduce a system, VitaLITy, intended to complement existing practices. In particular, VitaLITy promotes serendipitous discovery of relevant literature using transformer language models, allowing users to find semantically similar papers in a word embedding space given (1) a list of input paper(s) or (2) a working abstract. VitaLITy visualizes this document-level embedding space in an interactive 2-D scatterplot using dimension reduction. VitaLITy also summarizes meta information about the document corpus or search query, including keywords and co-authors, and allows users to save and export papers for use in a literature review. We present qualitative findings from an evaluation of VitaLITy, suggesting it can be a promising complementary technique for conducting academic literature reviews. Furthermore, we contribute data from 38 popular data visualization publication venues in VitaLITy, and we provide scrapers for the open-source community to continue to grow the list of supported venues.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> sections/old/case_study_old.tex <==
\section{Usage Scenarios: Bias in Visualization}
\label{sec:case_study}

\subsection{Motivation}
A common thread among the authors' prior research deals with \textbf{human bias in data visualization}, and in particular, the authors have focused on defining~\cite{wall2018four}, detecting~\cite{cho2017,WallBias,WallFormative,karduni2018can}, and mitigating~\cite{WallDesign} cognitive biases.
Through a number of prior discussions, we identified topics in visualization research that were relevant to our own work: e.g., Bayesian cognitive modeling~\cite{kim2019bayesian}, guidance~\cite{ceneda2017characterizing}, and mixed-initiative~\cite{Horvitz1999} visual analytics (e.g.,~\cite{BrownDisFunction2012,WallPodium,cook2015mixed}), to name a few.
However, seldom do authors of these topics utilize the language of \emph{bias}. 

Knowledge of these topics motivated the present work.
How could we identify these relevant topics in our literature reviews? 
A simple keyword search would not be fruitful due to a lack of common language. 
Thus, we find it fitting to put \system{} to the test in the domain of \textbf{bias in data visualization}.
In addition to identifying these known topics of interest, can our approach bring to light any additional topics of interest?



\subsection{Topics of Interest}
Prior to beginning our literature review, we identified three topics of interest we hoped our literature review would uncover: (1) Bayesian cognitive modeling, (2) guidance, and (3) mixed-initiative visual analytics. 

Bayesian cognitive modeling is often used in data visualization to compare how a user updates their beliefs in the presence of new and uncertain data to a normative benchmark~\cite{kim2019bayesian,karduni2020bayesian}. 
With respect to bias, this approach can be one promising direction toward characterization of bias (e.g., it can provide a normative framework in which to interpret observed user decisions).
While this approach has been recently proposed~\cite{wu2017towards}, to our knowledge it has not been used in empirical studies of bias in data visualization.

The topics of guidance and mixed-initiative visual analytics can similarly be relevant in the context of bias mitigation. 
These topics motivated a recent design space of bias mitigation techniques in visualization~\cite{WallDesign}.
In particular, techniques used to generally guide users through knowledge gaps in data analysis~\cite{ceneda2017characterizing} can be applied to guiding users toward a less biased analysis process. 
In doing so, systems are likely to employ mixed-initiative techniques~\cite{Horvitz1999} wherein systems assume some responsibility and control from users. 


\subsection{Strategy}
We began our search by ``blinding'' ourselves to the topics of interest. 
Hence, our search strategies were initially restricted to include use of ``obvious'' keywords (e.g., bias, decision making) and known papers on bias in visualization (e.g., the authors' own papers and select others that utilize the language of bias~\cite{dimara2017attraction,dimara2018task,dimara2019mitigating,gotz2016adaptive}). 


\subsection{Findings}

\subsubsection{Keyword Search}
global keyword search for ``bias'' returns 1639/59413 hits

given the scope of venues included, this revealed some relevant papers of interest (that likely would have been lost / difficult to filter for if searching via google scholar; less common venue, but still important for vis); 
- e.g., Two Implications and Dual-Process Theories of Reasoning. (venue: Diagrams)
- The Nudge Deck: A Design Support Tool for Technology-Mediated Nudging.(venue: Conference on Designing Interactive Systems)

Some of the usual suspects identified: 
- FairSight: Visual Analytics for Fairness in Decision Making.
- Selection Bias Tracking and Detailed Subset Comparison for High-Dimensional Data. (follow up paper to Gotz adaptive contextualization paper)
- Recent work on perceptual bias: Biased Average Position Estimates in Line and Bar Graphs: Underestimation, Overestimation, and Perceptual Pull.


\subsubsection{Similarity Search}

begin with my own paper~\cite{WallBias} as a seed
some obvious results:
- A Formative Study of Interactive Bias Metrics in Visual Analytics Using Anchoring Bias
- lots of DECISIVe hits (Cognitive Biases in Visualization book chapters)
- Adaptive Contextualization: Combating Bias During High-Dimensional Visualization and Data Selection.

some less obvious results: 
- Internalization, qualitative methods, and evaluation. (venue: BELIV)
- An Analysis of Machine- and Human-Analytics in Classification. (interestingly describes machine v. human+machine)
- Evaluating visualization using cognitive measures.
- Designing Theory-Driven User-Centric Explainable AI.
(can explanation techniques be used to mitigate bias in machine reliance?)
- Taking Development Seriously: Modeling the Interactions in the Emergence of Different Word Learning Biases.
- Bounded rationality leads to optimal decision-making and learning under uncertainty: Satisficing, prospect theory, and comparative valuation breaking the speed-accuracy tradeoff.
- BiDots: Visual Exploration of Weighted Biclusters.
- An Information-theoretic Framework for Visualization.



then adding my formative study paper and adaptive contextualization: 
- some weird ones come up: 
- A review of monocular visual odometry.
- Wall cavitation caused by projectile impact.

(by the end of the 25 output, we are getting similarity scores of 0)

then adding ~\cite{cho2017}, we get 
- Measuring Cognitive Load using Eye Tracking Technology in Visual Computing


new query: add all of my own papers as input to similarity search
output: User Evaluations of Interactive Multimodal Data Presentation. (suggests vis + sonification is promising...; this was actually rated really similar for some reason, interesting)
- Towards an instrument for measuring sensemaking and an assessment of its theoretical features. (sensemaking motivated a lot of my early work)
- Casual Information Visualization: Depictions of Data in Everyday Life. (I have since gone into some recent work on causality...)

tried similar query for each of us -- interestingly, similarity search based on all of our individual papers leads to some sensemaking papers for each of us (except Arpit, just based on the papers that are scraped of yours)


if we use ALL of our papers as input (20 in total): 
top 3 interestingly seem irrelevant: 
- Wall cavitation caused by projectile impact.
- BiDots: Visual Exploration of Weighted Biclusters.
- A review of monocular visual odometry.

Next ones seem better: 
- The Impact of User Characteristics and Preferences on Performance with an Unfamiliar Voice User Interface.
- Towards Deeper Understanding of User Experience with Ubiquitous Computing Systems: Systematic Literature Review and Design Framework.
- User Evaluations of Interactive Multimodal Data Presentation.
- Towards an instrument for measuring sensemaking and an assessment of its theoretical features.
- A Computational Model of the Role of Attention in Subitizing and Enumeration.
- Casual Information Visualization: Depictions of Data in Everyday Life.
- Effects of Sensemaking Translucence on Distributed Collaborative Analysis
- Trust in AutoML: exploring information needs for establishing trust in automated machine learning systems
- Demonstrational Interaction for Data Visualization.




\emily{- Not a gold standard by any stretch, but would be interesting to compare to the references captured in my (Emily)'s dissertation; I tried to be reasonably complete. What did I miss?}

%% Similarity Search by Papers
\begin{figure*}[!t]
    \centering
    \includegraphics[width=\linewidth]{figures/search-by-papers.pdf}
    \caption{Search by Papers. \arpit{To tweak to replicate the eventual bias case study.}}
    \label{fig:search-by-papers}
  \end{figure*}

%% Similarity Search by Abstract
\begin{figure*}[!t]
    \centering
    \includegraphics[width=\linewidth]{figures/search-by-abstract.pdf}
    \caption{Search by Abstract. \arpit{For this one, it'll be cool to do a search with our own final abstract that results in some similar papers that we actually cite in our related work.}}
    \label{fig:search-by-abstract}
  \end{figure*}

==> sections/old/study_old.tex <==
\section{Evaluation}
\label{sec:evaluation}

- evaluate the system via a case study comparison of our technique to an existing survey paper, perhaps Dimara's interaction paper~\cite{dimara2019interaction}


\subsection{Existing Survey Methodology}

- in addition to systematic lit reviews conducted for papers, we also examined several survey papers (e.g., ~\cite{})
- these surveys describe their methodology for lit reivew, including collecting an initial set of seed papers, keyword search, inclusion criteria, venues considered, etc.


\subsection{Existing Survey Results}

- total number of papers found, high level topics covered


\subsection{Our Survey Methodology}

- need to give our system a catchy name to refer to it here ;) 

- describe our alternative approach, including both keyword and exemplar paper search


\subsection{Our Survey Results}

- total number of papers found, clusters of topics that formed



\subsection{Comparing Survey Results}

- using two alternative methodologies, we achieved (hopefully at least close to) comparable results using less manual effort

- set comparison: if the Dimara survey is set A and our survey is set B, how many papers are in the intersection? how many in the set difference A-B and B-A? 

==> sections/old/user_feedback.tex <==
\subsubsection{Positive Quotes}

- searching nearby papers in the embedded space, after lassoing: S01 said “This is interesting. It seems there are some papers here that might be useful.”
“I feel like I would spend a lot of time on this. It’s like this mystery, I feel like if I spent some time on this, I might stumble upon a paper that was relevant that was published in a different domain. And that’s basically like half of the papers that I cite.”
“It might be especially useful if I worked on a different topic that I hadn’t worked on in the past.”

- Search by abstract: S01 said “If I’m starting a new project and I don’t know if this has been done, I can write up some words in the form of an abstract to see if this is done.”

- would you use this? S01 “Yeah, I think it could be very useful if I have a gap in my lit search. There are some papers I should cite, and if i don’t cite them, then reviewers will be like ‘you should cite these papers’, and this seems like it would yield such results. I have some confidence. This garden of forking paths paper I had not search for but it came up because of this similarity search. And if I were in a new domain where I didn’t have a lot of background knowledge, this would be useful. I would interleave this with a Google Scholar search. If I found a few relevant papers, I would go to Google Scholar to see the references in that paper and who has cited that paper. And that’s a workflow that I’m familiar with.“

- would you use this: S02 “I can see myself using a tool like this, especially for someone like me who has been in the field for a bit and knows where to begin the search process. But I wish fine tuning search results were more intuitive. I could find some relevant papers, then use the JSON output to reduce the search space within another tool like Google Scholar.”

- specter embeddings: S02, after less successful 2-D search w/ glove: “I’m going to try 2-D search with Specter. This search seems to be a little bit better.”

- favorite features: S02 “I think the table view at the top is a really good starting point. It works really well. It shows the authors, etc. that I expect to see. It’s a good entry point for the user. The saved paper cart is also a neat addition. I will always be mindful of my goal to fill the cart with relevant papers.”

- in response to keyword search results, S03 “I’ve read this one before [Verifi]. This one I don’t care about, it’s more machine learning. I’d like to find more social science.” 
“Social Media… sounds interesting, I want to save this paper to read it later.”
“Nudging, this is interesting. I should take a look at the abstract.”
“Now I just want to check out the other papers from this author“ [Zhicong Lu]
“I think I’ll read some of these.”

- saved paper cart: S03 “I liked the fact that I’m able to save some of the papers. Typically I wouldn’t do it that way. When I search for papers that might be relevant, I just use a word document or something to keep track of the titles and maybe download the paper as well. It’s nice to be able to save the papers.”

- after doing n-D similarity search, S04: “Ohhh, interesting, I never knew that these two people had a collaboration.” -- in response to interesting relevant network paper [Cody Dunne and Ben Shneiderman]

- S04 “I liked the visualization, especially the lasso select. It’s really cool and really helpful.” 
“Also, locate is a really good feature, you can actually identify the papers in different colors.”

- would you use it? S04 “I definitely see myself using this app. I really like the idea of this visualization, it’s really cool, because it’s very helpful to actually find a set of papers that are semantically relevant to one paper. Especially when I can randomly identify a paper that I missed in the lit review, and find other papers similar to that one to be sure you aren’t missing anything.“

- relevance of similarity output: S05 “The papers I’m seeing now are a lot more relevant, some of the papers I’ve been reviewing. Hmm, some of them are kind of new, but let’s see if they’re relevant to my topic.”
“I’m trying to find if there are new papers worth exploring.”
“This one seems interesting, so I would like to add this to my list and maybe save it as well.”

- found something really similar to what she was thinking of writing about: S05 “I’m noticing some papers that I was considering to review to write my discussion section. I wanted to review other related domains and use this analytical framework to conduct research in that domain. One possibility was to use it for evaluations of different structures of storytelling visualizations. I’m seeing a paper that did something similar to what I was considering doing.”

- S05 “I want to see 2-D similarity results now -- ohh, this is interesting: Design Patterns for Data Comics.”

- distinction between 2-D and n-D similarity: S05 “I do see a difference, I think 2-D search may be giving me more relevant results.” 
“Might be better for more in-depth exploration. If there’s a very specific topic you’re looking for. For example, I was looking for analytical frameworks within storytelling. And it seemed like 2-D similarity search gave better results.”
“n-D seemed to give better results that were exploratory. I found some interesting papers I would like to read more.” 

- S05 “This was actually useful, because there were some papers that caught my eye that I hadn’t seen before.”

- similarity search S05 “I really liked the similarity search. I liked that you showed the similarity score. It seems reasonable… Those on top tended to be more relevant to what I was looking for.”

- umap S05 “I guess this [umap] provides a nice overview of the selected papers, and I could see to drill down into more details or look for clusters.”

- would you use it? S05 “Yes. I would probably use it when I have some high-level ideas about how I would structure the related sections -- when I know what those 2-3 themes are. I would use this to find more relevant papers.”

- S06: Hid author column and resized column to see full titles… seemed very intuitive to him, he expected it would do this

- Appropriation of abstract search: S06 after searching in abstracts, applying filters for relevant venues, etc. felt unsatisfied by results; so used search by abstract instead: “Maybe I should use word embedding because it might have more flexibility and I can pass more information in my search.” 
“It shows a lot of foundational literature…”
[after first iteration results were only ok, added more content to the abstract and was much more satisfied with results]
“Wow, this shows much better results now than the short abstract.”
“Presentation-oriented visualization techniques -- hmm looks interesting.”
“Oh this looks interesting, but I haven’t looked at.” [Comparing the Effectiveness of Visualizations of Different Data Distributions]
“I should take a note.” [writes down paper info]
“This one, I think I cited this one.”
“I’m also writing down this one. It’s look at EEG, wow. It looks interesting because I cited a similar mathematical paper, they want to approximate the same thing.” [Comparing Similarity Perception in Time Series Visualizations]

- satisfaction w/ search: S06 “Yes, I was mostly looking for papers that I haven’t looked at before. For 15 minutes, I found two papers I might be interested in. It’s a really useful process. Otherwise I might spend a lot of time scanning PDFs, which is not a very pleasant experience.”

- lots of good features: S06 “Search by abstract was super useful. Personally I’m not super familiar with these visualizations, dimensionality reduction, so it’s harder to interpret how to assess this information.”
“The similarity measures here [in similarity output] were really useful. But some would return like 0.0001 and I could see that my search was wrong.”
“For lasso selection, I want to see factors that can cluster similar papers. I want to just see similarity output, not select everything.” 
“Changing columns was useful too, so I can get a better sense of the data. If the search gets improved then search by abstract will be much better. Google Scholar searches body text too. But for Google Scholar the similarity [or relevance?] of results is not so good.”

- when it's useful (at the end of lit review) S06: “For searching papers, I would continue to use Google Scholar when I start the lit review. But I think vitaLITy could be super useful at the later stage of your research. You want to do some sanity checks on your literature review. At that point of time, I have my abstract, more details, papers I have already cited, and based on that, I can do a more narrow search for papers I might be missing. When you’re finalizing your literature review. It can help people evaluate their process and understand how they are doing, how they can improve. Sometimes you get reviews that you didn’t cite this or this or this and it’s sort of embarrassing.”





\subsubsection{Negative Quotes} 
- in reasoning about the quality of similarity output: “I see why these papers are not giving the best results. It seems in the word embedding space, they are not close together.” (S01)
- did you find useful papers: S01 said “I could find a few papers that came up that slipped my mind. But I didn’t find any new papers that I hadn’t already cited. I got some sense that the search was giving me useful results. I have some confidence that it would work, but for this particular context, I did not find anything new.”

- some resistance to doing things a different way: S01 said “I’m having some of the same difficulties that I have when I do a Google Scholar search. I need to find one paper. My target is one unknown paper among hundreds. It’s very rare that I find multiple useful papers when I try random keywords on Google Scholar. A lot of the papers I find because coauthors tell me about a relevant paper. A lot of the papers that we cite are not directly relevant, but it’s adjacent. That kind of makes it complicated to search if I had already filtered on a particular keyword.”
- S03 “I prefer Google Scholar. Would I use it? Maybe… I suspect I would use it just like I use Google Scholar. I wouldn’t use similarity search. I would just search for keywords. I’m not sure how Google Scholar does it, but I like this global search to look in abstracts, titles, etc.”

- didn't use umap much: S01 "This visualization [scatterplot] was interesting, but I spent very little time on this. I’m not sure why, but it almost seemed like I would need very specific input to find relevant results, so I ended up spending more time on filtering that I would want a similarity search on."

- relevance of glove output: S02 “The original paper I’m looking for Regroup, these do not seem to be good results. The 2-D search does not seem to be good with Glove. The n-D results were much better.” [switched to specter], “Maybe if I give a few other papers as examples, it may help.” [adds 2 more papers]
“Some matches, but some do not.”
- S05 “I’m reviewing the results, some seem relevant, some not so much.”

- quality of similarity search results: S02 “When I look by author or keywords, I find relevant papers. But when I try to fine tune, it loses track. I could have expected better search results.”

- accuracy / utility of umap projection, S03 “not sure these are so similar” -- appear far apart (did n-D search rather than 2-D)
 “I don’t think I need to see all the papers at once. I mostly want to see all the papers I have selected and their geolocation and whether they’re similar or not so similar. But the algorithm might be bad. Or the projection. It doesn’t accurately depict similarity between papers.”
 
 - too much packed into one tool: S04 “The unique part of this interface is the visualization of the space of papers. I wish it could be bigger canvas space so I can select papers. The interface is a little small and too compact that makes me feel like too many things are changing in front of my face and I lost track.”
“I feel like the similarity search and visualization can be a separate thing on its own. And the meta thing and table search can be on its own.”

- didn't use saved papers cart S06: “I realized looking at the questions that I never used the saved papers cart. Even using Google Scholar I usually just prefer to save the PDF.”





\subsubsection{Desired Features} 

- citation networks: S01 “The other thing, in this case, I forgot to mention this, but a way I conduct literature reviews is to look at the cited papers of a relevant paper and then go in a search. That is missing. Google Scholar makes it easier, but it’s not great.”
- S06 “I think it’s hard to implement, I’ve tried it before, but maybe it could show the citation map. Sometimes I find a really old paper that has some really core ideas and I want to see more recent papers that cite it.”

- more embedding options: S02 
“Other than Glove, you can consider to use transformer embeddings like BERT. It uses context vectors.”

- indicators about credibility of venue / author: S03 "If I’m able to get a sense of how credible the source is, e.g., this particular conference. When it comes to some other domains or venues, we have a hard time getting an indicator of whether this is a good conference or not until we read the paper, or if we know the author is highly cited and respected.”

- alternate way to visualize umap: S04 “Is there any possible way to visualize this in terms of networks? If you can separate out the nodes in space and add edge weights to reflect similarity. The biggest problem is overlapping nodes, so I don’t have a full picture. Or at least put the red dots in the top layer. Now you have three layers: filtered, unfiltered, saved. Maybe I can use the legend as a filter to show only that layer.”

- metal panel integration: S04 “I didn’t feel like I used the meta panel a lot. Is it possible that I select a keyword that it could query all papers that have this keyword in the search / umap?”

- suggested keywords: S05 “For keywords, if I could look for multiple keywords…”
“Can it suggest semantically similar keywords?”



\subsubsection{Small Usability Issues}

- fuzzy string search could be useful: S01 searched for "uncertainty visualisations" -> "uncertainty visualizations" -> "uncertainty visualization" 
- S01 also tried multiple keywords; may be beneficial to have more robust and customizable search mechanism
- SOMEONE used the search by abstract as a workaround (interestingly)

- "Wall Cavitation" paper seems to come up frequently (in our usage scenarios and in participant sessions) [I think just for Glove?]; something about abstract length (very short) makes it seem like a good match for lots of searches

- feedback about queries: S01 “I did find a lack of feedback on the queries.”
S05: “Apart from being a little laggy, it was pretty straightforward. But I kept forgetting to clear out the search [clear filters].”

- customizable layout: S02 “I found myself when I had already filtered by keywords, I am only focusing on this view [scatterplot], it’s very small in the screen space. I want to hide the meta view and maybe even the main table view, so I can easily zoom and pan and lasso. The similarity search panel could also be bigger.”
- S04: “I wish this interface [umap] could be a little bigger.”
- S06 “I think the window [top table] is a little bit short. Can I expand this?” [no, could not... although was able to very intuitively resize / customize column widths]

- zoom level on umap: S02 “When I do this similarity search, it should automatically zoom to show the paper(s) that were the beginning search point and the papers that it found, rather than this zoomed out view where I have to look for the orange or red dots.”

- button layout: S02 “The glove / specter and n-D / 2-D buttons should be closer together so it’s easier for me to realize where to make changes related to the search process.”

- keywords in meta view: S03 “Keyword feature can be useful if it’s not displaying keywords for the stuff above but for what I have selected.”

- S06 “Most of the features were really good as-is.” 
“Maybe the interface might be able to support more natural interactions -- more connected between these panels. E.g., if I filter keyword here [meta view] it would filter here [main table].”
“When I search the abstract, it might be useful to support non-exact match, because you usually don’t expect an exact string match.”
“Match the conferences were not matched -- like 20 Eurographics [variations].”
“Some focus on sections. If I’m working on the table, this could be bigger, or let users change the proportion of the panels.”


==> tables/venues.tex <==
\setlength\tabcolsep{3pt} % default value: 6pt
\begin{tabular}{llll}
    \hline
    \multirow{1}{*}{IUI} & 
    \multirow{1}{*}{UIST} &
    \multirow{1}{*}{VAST} &
    \multirow{1}{*}{SIGGRAPH} \\ 

    \multirow{1}{*}{VIS} &
    \multirow{1}{*}{TCHI} &
    \multirow{1}{*}{IVAPP} &
    \multirow{1}{*}{INTERACT} \\

    \multirow{1}{*}{ICS} &
    \multirow{1}{*}{SciVis} &
    \multirow{1}{*}{EuroVIS} &
    \multirow{1}{*}{Cognitive Science} \\

    \multirow{1}{*}{AVI} &
    \multirow{1}{*}{ICDM} & 
    \multirow{1}{*}{SIGMOD} &
    \multirow{1}{*}{Graphics Interface} \\

    \multirow{1}{*}{CHI} & 
    \multirow{1}{*}{TVCG} &
    \multirow{1}{*}{SIBGAPI} &
    \multirow{1}{*}{The Visual Computer} \\

    \multirow{1}{*}{CGF} & 
    \multirow{1}{*}{BioVis} &
    \multirow{1}{*}{BCS HCI} &
    \multirow{1}{*}{Cognitive Biases in Vis.} \\

    \multirow{1}{*}{CGA} &
    \multirow{1}{*}{CSCW} &
    \multirow{1}{*}{Diagrams} &
    \multirow{1}{*}{Journal of Visualization} \\

    \multirow{1}{*}{KDD} & 
    \multirow{1}{*}{VCBM} &
    \multirow{1}{*}{UbiComp} &
    \multirow{1}{*}{Information Visualization} \\

    \multirow{1}{*}{VMV} &
    \multirow{1}{*}{BELIV} &
    \multirow{1}{*}{PacificVis} &
    \multirow{1}{*}{Designing Interactive Systems} \\

    \hline
\end{tabular}%
